Content-aware Tile Generation using Exterior Boundary Inpainting

We present a novel and flexible learning-based method for generating tileable image sets. Our method goes beyond simple self-tiling, supporting sets of mutually tileable images that exhibit a high degree of diversity. To promote diversity we decouple structure from content by foregoing explicit copying of patches from an exemplar image. Instead we leverage the prior knowledge of natural images and textures embedded in large-scale pretrained diffusion models to guide tile generation constrained by exterior boundary conditions and a text prompt to specify the content. By carefully designing and selecting the exterior boundary conditions, we can reformulate the tile generation process as an inpainting problem, allowing us to directly employ existing diffusion-based inpainting models without the need to retrain a model on a custom training set. We demonstrate the flexibility and efficacy of our content-aware tile generation method on different tiling schemes, such as Wang tiles, from only a text prompt. Furthermore, we introduce a novel Dual Wang tiling scheme that provides greater texture continuity and diversity than existing Wang tile variants.

==> fig_classic.tex <==

\begin{figure}[t!]
  \begingroup
  \setlength{\fboxrule}{2pt}
  \setlength{\fboxsep}{0pt}
  \fbox{\adjincludegraphics[width=\columnwidth-2\fboxrule,trim={0 {0.5\height} 0 0},clip]{classic_strict_wang.large.png}}
  \endgroup
  \caption{Compared to~\autoref{fig:comparison} (2nd row, 1st column),
    graph-cut based synthesis of the Wang tile textures yields less
    texture diversity.}
  \label{fig:classic}
\end{figure}


==> fig_classic_flowers.tex <==

\begin{figure}[t]
  \begingroup
  \setlength{\fboxrule}{2pt}
  \setlength{\fboxsep}{0pt}
  \fbox{\adjincludegraphics[width=0.5\columnwidth-5\fboxrule]{orange_lily.large_classic_wang.png}}
  \endgroup
  \caption{The graph-cut based synthesis of the Wang tile textures yields less
    texture diversity.}
  \label{fig:classic}
\end{figure}

